AgentDSE: Reasoning-Augmented Architectural Design Space Exploration

Traditional architectural design space exploration (DSE) is highly inefficient, typically requiring tens of thousands of simulator evaluations across various optimization methods. This inefficiency arises because conventional methods treat the simulator as a black-box oracle. In contrast, human architects effectively guide exploration by reasoning through physical constraints, performance bottlenecks, data reuse, and workload structures. To bridge this gap, we introduce AgentDSE, a simulator-in-the-loop methodology driven by a general-purpose large language model (LLM) coding agent. AgentDSE automates this architectural-reasoning loop without requiring model fine-tuning, precomputed design databases, or domain-specific optimizer code. Across deep neural network (DNN) accelerator mapping, hardware/software co-design, and CPU cache-hierarchy optimization, AgentDSE achieves competitive or better design quality with up to two orders of magnitude fewer evaluations. AgentDSE also produces inspectable traces that surface architectural hypotheses, performance cliffs, implicit priors, and simulator artifacts, making every search decision traceable rather than buried in optimizer state.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Agent--Simulator Interface}
\label{sec:background:interface}

Our goal is to study whether a coding agent can act as a simulator-in-the-loop design space explorer.
To make this setting concrete, we represent each DSE problem as a self-contained workspace.
The workspace contains: (1) a task description specifying the objective and budget; (2) an action-space specification describing valid design parameters and constraints; (3) mutable candidate files that encode the current design point; and (4) a submission script that evaluates the candidate through the target simulator and returns the resulting metrics.
Optionally, the workspace also includes a notebook-like file for recording intermediate hypotheses and observations.

This interface deliberately separates the \emph{optimizer} from the \emph{evaluator}.
The coding agent is responsible only for proposing and revising candidate designs, while correctness and performance are determined entirely by the underlying simulator.
As a result, the same optimization workflow can be reused across domains as long as the task can be expressed through editable candidate files and a callable evaluation script.

\subsection{Coding-Agent Optimization Loop}
\label{sec:background:loop}

Unlike one-shot prompting, a coding agent operates through an iterative read--edit--run loop.
At each step, the agent reads the current workspace state, edits the candidate design, executes the submission script, inspects the returned metrics, and revises its next proposal accordingly.
This makes optimization an explicit hypothesis--evaluate--refine process rather than a sequence of isolated simulator calls.

A useful byproduct of this interface is traceability.
Because the agent interacts through files and tool calls, its search process can be logged as a sequence of intermediate hypotheses, candidate edits, simulator outputs, and subsequent refinements.
In this paper, we use these traces not only to measure final design quality, but also to analyze why the search succeeds or fails, and to identify reward hacks or simulator artifacts that would be difficult to diagnose from scalar optimization curves alone.

\subsection{Target DSE Settings}
\label{sec:background:domains}

We evaluate the same agentic workflow across three qualitatively different DSE settings.

\textbf{MAESTRO.}
MAESTRO~\cite{kwon2019maestro} is used for DNN accelerator mapping, where the search space includes loop order, tiling factors, spatial mapping dimensions, and PE allocation.
The objective is to minimize energy-delay product (EDP) for a fixed hardware target and workload.

\textbf{Timeloop+Accelergy.}
Timeloop~\cite{timeloop} together with Accelergy~\cite{accelergy} supports accelerator hardware/software co-design.
Compared with mapping-only search, this setting jointly explores hardware parameters and mappings, yielding a broader design space and providing a natural testbed for comparison against differentiable DSE.

\textbf{ChampSim.}
ChampSim~\cite{champsim} is used for CPU cache-hierarchy DSE, where the search space includes cache sizes, associativities, replacement policies, prefetchers, and branch predictors under hierarchy and area constraints.
The objective is to maximize IPC on representative SPEC CPU workloads.

Although these three settings differ substantially in simulator stack and design semantics, they share the same optimization interface: a candidate design is written to a file, evaluated by a simulator, and returned as numeric feedback under domain-specific validity constraints.
This common structure is what enables a single coding-agent workflow to be reused across simulator families.

==> backup_discussion.tex <==
\section{Discussion and Limitations}

\textbf{Cost.}
Each 100-call \sysname{} run consumes approximately 200K tokens (\$1--2 at current API pricing).
This is negligible compared to the engineering time saved, but non-trivial for large-scale sweeps.
Using smaller models (e.g., Sonnet) or distilled prompts could reduce cost.

\textbf{Reproducibility.}
LLM outputs are stochastic.
Across two independent runs on the BERT task, both converged to the same optimal action (EDP = 1.99$\times10^9$), but at different call counts (call 65 vs.\ call 3).
Systematic reproducibility studies across more seeds are needed.

\textbf{Scaling to larger design spaces.}
Our 15-dimensional MAESTRO action space is moderately sized.
Whether the approach scales to 50+ dimensional spaces (e.g., full chip floorplanning) remains an open question.

\textbf{Simulator fidelity.}
As noted in Section~\ref{sec:audit-limit}, the agent can exploit simulator artifacts.
This is both a strength (detecting reward hacks) and a limitation (results may not transfer to real hardware without artifact-aware evaluation).

\textbf{Prompt-engineering as an unstated baseline.}
Our \texttt{action\_space.md} contains hand-distilled hardware-architecture priors (per-knob semantics, per-workload heuristics, an example config). Removing these and re-running \sysname{} would isolate ``coding agent'' from ``coding agent + curated prior.'' We have not yet performed this ablation; the reported numbers are conditional on the prompt as written. A purely zero-shot variant (schema-only prompt, no heuristics) is the most informative single follow-up experiment for the methodology claim.

\textbf{Statistical thinness.}
We use $n=3$ seeds per (workload, method) and report point estimates. Within-seed variance (different Claude initializations sampling the same workload) appears to be small empirically (e.g., the three CC seeds on mcf all converged to IPC = 0.6141), but we have not computed Wilcoxon signed-rank tests, bootstrap CIs, or $p$-values, and 3 seeds is the floor of what is defensible. Some of the smaller margins we report (e.g., 0.34\% on mcf, 0.9\% on omnetpp) are below the noise floor of our 5\,M-instruction simulation window and should be interpreted as ties.

\textbf{Simulation-window length.}
ChampSim runs use 1\,M warmup + 5\,M simulation instructions, two orders of magnitude shorter than the DPC-3 / Championship-Prefetching standard (200\,M warmup + 500\,M sim). We expect the relative ranking among methods to be stable at longer windows, but the small (sub-1\%) gaps we report can swing under longer simulation; re-evaluating the top-3 designs per method at full window is the verification step that completes this experiment.

\textbf{Garden-of-forking-paths.}
Two design choices were made post-hoc on this dataset: the L1D~$\le$~L2C~$\le$~LLC hierarchy constraint was added after we observed implausible inverted-hierarchy samples in the random/GA/BO histories, and the 4.5\,MiB area budget was chosen to make the LLC/L2 trade-off a meaningful decision under the hardware. Both choices were made without observing per-method best-IPC outcomes, but the audit-style critique applies; we report the unfiltered numbers in the lab notebook for transparency.

\textbf{Cross-domain claim, scoped honestly.}
ChampSim cache DSE is densely covered by Claude's training data (the SPP, SHIP, and DPC-3 papers we benefit from are public and indexed). The honest reading of our generalization result is that the \sysname{} \emph{methodology} (workspace + agent loop) transfers from MAESTRO to ChampSim using the same code path with no per-domain custom logic, not that the agent has been demonstrated to perform open-domain hardware reasoning. The next test—and a stretch goal for a journal version—is a domain Claude has weak prior on (NoC topology, DRAM controller policies, or a synthetically obfuscated DSE).


==> backup_exp.tex <==
\section{Experimental Setup}
\label{sec:setup}


\textbf{Simulator.}
We evaluate mappings with MAESTRO~\cite{kwon2019maestro}, a data-centric cost model for DNN accelerator dataflow mapping.
Each evaluation generates a MAESTRO mapping file, invokes the simulator, and parses runtime cycles and activity-count energy from the generated CSV output.

\textbf{Hardware target.}
We use a memory-constrained accelerator configuration inspired by edge-class DNN accelerators~\cite{eyeriss}.
The configuration provides a two-level memory hierarchy with a 256B L1 scratchpad, a 64KB shared L2 buffer, 64 bytes/cycle NoC bandwidth, and 32 bytes/cycle off-chip bandwidth.
The design space also includes the effective number of PEs allocated to the mapping, with valid values in $[4,1023]$.
This setting stresses mapping quality because the small on-chip memories force aggressive tiling and expose off-chip traffic penalties.

\textbf{Workloads.}
We evaluate 10 GEMM shapes from two production-scale AI models.
Each GEMM is represented in MAESTRO as a $1{\times}1$ convolution with dimensions $(K,C,X,Y=1,R=1,S=1)$.

\begin{itemize}[leftmargin=*,itemsep=1pt]
    \item \textbf{LLaMA-3.1-8B}~\cite{llama3}: 4 unique shapes from a transformer block: Q/O projection, K/V projection under GQA, FFN gate/up projection, and FFN down projection. These occur 32--64 times across the 32-layer model.
    \item \textbf{OpenVLA}~\cite{openvla}: 6 unique shapes from the DINOv2-L vision encoder and the LLaMA-2-7B action backbone. The DINOv2-L encoder contributes Q/K/V/O, FFN-up, and FFN-down shapes across 24 layers; the action backbone contributes Q/K/V/O, FFN gate/up, and FFN-down shapes across 32 layers.
\end{itemize}

\textbf{Methods.}
All methods use the same MAESTRO evaluation interface, hardware configuration, and 15-dimensional integer action space over dataflow order, L1/L2 tiling, spatial mapping dimensions, and PE allocation.

\begin{itemize}[leftmargin=*,itemsep=1pt]
    \item \textbf{Random Search (RS)}: 20,000 uniformly sampled actions.
    \item \textbf{Genetic Algorithm (GA)}: population size 50, tournament selection with size 3, uniform crossover with probability 0.8, mutation rate 0.2, elitism over the top 2 individuals, and 20,000 evaluations.
    \item \textbf{PPO (single-agent)}: a lightweight MLP policy with two 128-unit hidden layers. The policy samples a continuous action in $[-1,1]^{15}$, which is discretized to valid MAESTRO action ranges, and is trained for 50,000 evaluations using reward $-\log(\mathrm{EDP})$.
    \item \textbf{\sysname{}}: Claude Code CLI via \texttt{claude -{}-print}, given the same task files and a 100-call MAESTRO budget.
\end{itemize}

\textbf{Metric.}
The objective is Energy-Delay Product, $\mathrm{EDP}=\mathrm{runtime\ cycles}\times\mathrm{energy\ nJ}$.
For each unique GEMM shape, we report the best valid EDP found within the evaluation budget.
When reporting model-level results, we aggregate shape-level EDP using the workload multiplicities:
$\sum_i \mathrm{EDP}_i \times \mathrm{count}_i$, where $i$ indexes unique GEMM shapes.
%% ===================================================================
\section{Results}
\label{sec:results}

\subsection{Per-Shape Comparison}

Table~\ref{tab:per-shape} shows the best EDP achieved by each method on all 10 GEMM shapes.
\sysname{} wins 8 out of 10 shapes despite using 200--500$\times$ fewer simulator calls than the baselines.

\begin{table}[t]
\small
\caption{Best EDP by method across 10 GEMM shapes on Config-C hardware (512 PEs, 256B L1, 64KB L2). Bold = best per shape. \sysname{} uses 100 calls; RS/GA use 20K; PPO uses 50K.}
\label{tab:per-shape}
\centering
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Model} & \textbf{Shape} & \textbf{\sysname{}} & \textbf{RS} & \textbf{GA} & \textbf{PPO} \\
 & & \textbf{(100)} & \textbf{(20K)} & \textbf{(20K)} & \textbf{(50K)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize LLaMA-8B}}
& Q/O proj  & \textbf{2.9e13} & 6.7e13 & 3.7e13 & 3.1e13 \\
& K/V proj  & \textbf{4.3e12} & 7.4e12 & 7.3e12 & 4.9e12 \\
& FFN up    & \textbf{2.6e14} & 5.2e14 & 2.7e14 & 2.7e14 \\
& FFN down  & \textbf{2.8e14} & 1.5e15 & 3.5e14 & 3.1e14 \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize DINOv2}}
& QKVO      & 6.7e9  & 8.3e9  & \textbf{5.7e9}  & 6.8e9  \\
& FFN up    & 9.2e10 & 1.0e11 & \textbf{6.1e10} & 7.1e10 \\
& FFN down  & \textbf{6.5e10} & 6.9e10 & 1.6e11 & 7.7e10 \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize LLaMA-2}}
& QKVO      & \textbf{1.1e13} & 2.1e13 & 1.2e13 & 1.2e13 \\
& FFN up    & \textbf{6.0e13} & 1.7e14 & 6.1e13 & 6.5e13 \\
& FFN down  & \textbf{6.0e13} & 1.8e14 & 7.4e13 & 7.4e13 \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Model-Level EDP}

Table~\ref{tab:model-edp} shows the weighted model-level EDP.
On LLaMA-3.1-8B, \sysname{} achieves the \textbf{best overall EDP} with only 100 calls per shape (400 total for 4 unique shapes), outperforming PPO at 50K calls per shape.

\begin{table}[h]
\small
\caption{Model-level weighted EDP ($\sum \text{EDP}_i \times \text{count}_i$). Lower is better.}
\label{tab:model-edp}
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model} & \textbf{\sysname{}} & \textbf{RS} & \textbf{GA} & \textbf{PPO} \\
 & \textbf{(100/shape)} & \textbf{(20K)} & \textbf{(20K)} & \textbf{(50K)} \\
\midrule
LLaMA-3.1-8B & \textbf{2.80e16} & 8.57e16 & 3.09e16 & 2.94e16 \\
OpenVLA      & 5.75e17 & 1.90e16 & \textbf{7.83e15} & 8.03e15 \\
\bottomrule
\end{tabular}
\end{table}

On OpenVLA, \sysname{} is dragged down by a single catastrophic failure on the LLaMA-2 FFN-down shape (EDP 1.8e16 vs.\ GA's 7.4e13---a 240$\times$ gap).
We analyze this failure mode in Section~\ref{sec:ablation}.

\subsection{BERT Baseline (Prior Work Comparison)}

On the BERT-base Q-projection (K=C=768, X=512) with the production MAESTRO configuration (1GB L1/L2, unconstrained bandwidth), \sysname{} achieved EDP = 1.99$\times10^9$ in 100 calls, surpassing the MARL B=3 system's best of 2.88$\times10^9$ after 50,000 steps---a 31\% improvement with 500$\times$ fewer evaluations.
At the reward threshold of $-23.0$ (-log EDP), \sysname{} reached it in 6 calls versus MARL's 13,600 steps, a \textbf{2,267$\times$ sample efficiency advantage}.

\subsection{Ablation: Failure Mode Analysis}
\label{sec:ablation}

\sysname{}'s failure on the OpenVLA LLaMA-2 FFN-down shape (K=4096, C=11008, X=2048) reveals a systematic limitation.

\textbf{Root cause: spatial dimension bias.}
The agent consistently attempts to spatialize the K dimension (4096), which is the output dimension and typically the better choice for square GEMMs.
However, FFN-down is highly non-square (C/K = 2.69), and the optimal mapping spatializes C (11008) instead.
The agent's domain knowledge contains a ``default to K-spatial'' heuristic that is correct for 8/10 shapes but catastrophically wrong for this one.

\textbf{Comparison with GA/PPO.}
GA and PPO, lacking this heuristic bias, explore both K-spatial and C-spatial configurations uniformly and find the C-spatial optimum within their larger budgets.
This illustrates a fundamental tension: \emph{domain knowledge enables sample efficiency but can introduce systematic bias}.

\textbf{Mitigation.}
Increasing \sysname{}'s budget to 200 calls or adding an explicit ``try all spatial dimensions'' directive to the prompt could address this.
We leave systematic prompt engineering for robustness to future work.

%% ===================================================================
%% Auto-updated from experiments/cc-dse-v2/exp_dosa_compare_001/scripts/aggregate_results.py
\input{exp_dosa_compare_001_results.tex}

%% ===================================================================
\section{Cross-Domain Generalization: ChampSim}
\label{sec:additional}

A natural concern with the MAESTRO results is that DNN-mapping is a heavily-studied domain in Claude's training data---the agent may be reciting well-known dataflow tropes (weight-stationary, output-stationary, KCP) rather than performing genuine search. We test cross-domain generalization on a fundamentally different architecture-DSE problem: CPU memory-hierarchy design with the trace-driven ChampSim simulator~\cite{champsim}. Different simulator, different objective (IPC, not EDP), different action format (categorical + log-spaced sizes, not loop-tile vectors), different workload class (SPEC CPU integer/FP programs, not DNN layers), and different constraint regime (aggregate area + monotonic cache hierarchy, not loop-tile feasibility).

\subsection{Setup}

\textbf{Simulator.} ChampSim simulates a single-core out-of-order CPU with a 3-level cache hierarchy. Each evaluation compiles ChampSim with a candidate config, runs a SPEC CPU2017 trace (1\,M warmup + 5\,M simulation instructions), and reports IPC. Builds and simulations are isolated inside per-worker podman containers based on a self-contained ChampSim image (built once, replicated across compute nodes), eliminating shared-filesystem build races.

\textbf{Search space.} The agent chooses, for each cache level, the number of sets, ways, replacement policy, and prefetcher; plus a branch predictor. The Cartesian product is $\sim$708\,M configurations; after enforcing a 4.5\,MiB SRAM area budget and an L1D~$\le$~L2C~$\le$~LLC hierarchy constraint, $\sim$293\,M remain feasible. Concretely the agent chooses among \{32, 64, 128, 256\} L1D sets and \{4, 8, 12, 16\} ways; \{lru, srrip, drrip, ship\} for replacement at each level; \{no, next\_line, ip\_stride, va\_ampm\_lite, spp\_dev\} for prefetchers (subset per level); \{bimodal, gshare, hashed\_perceptron, perceptron\} for the branch predictor.

\textbf{Workloads.} Three SPEC CPU2017 traces chosen for memory-behavior diversity:
\begin{itemize}[leftmargin=*,itemsep=1pt]
    \item \texttt{605.mcf\_s}: pointer-chasing through a large in-memory graph; latency-bound, hostile to prefetchers, sensitive to LLC capacity and replacement policy.
    \item \texttt{619.lbm\_s}: streaming Lattice-Boltzmann fluid simulation; bandwidth-bound, prefetcher-friendly, working set dwarfs any feasible LLC.
    \item \texttt{620.omnetpp\_s}: discrete-event network simulator with mixed object/heap activity and irregular pointer access.
\end{itemize}

\textbf{Methods.} All four methods write a candidate to \texttt{candidate.yaml} and call the same \texttt{eval.py} (which dispatches to a per-worker container). \sysname{} runs Claude Code as in MAESTRO; \textbf{Random} samples uniformly with area+hierarchy rejection; \textbf{GA} is a per-worker micro-GA (pop=10, tournament=3, elitism=2, mutation=0.15, uniform per-field crossover); \textbf{BO} uses a random-forest surrogate (50 trees) with UCB acquisition (k=1.5) after 15 random warm-start points.

\textbf{Replication.} 3 SPEC traces $\times$ 3 seeds $\times$ 4 methods. \sysname{} self-terminates around $\sim$50 calls per run; the three gradient-free baselines are forced to use a budget of \textbf{1000 calls} each---more than 20$\times$ \sysname{}'s.

\subsection{Results: sample efficiency and IPC}

\begin{table}[t]
\small
\caption{Best IPC by method across 3 ChampSim workloads. \sysname{} self-terminates around 50 calls; Random/GA/BO are forced to 1000 calls each. Numbers are mean across 3 seeds, hierarchy-filtered. Bold = best per row.}
\label{tab:champsim-per-workload}
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Workload} & \textbf{\sysname{}} & \textbf{Random} & \textbf{GA} & \textbf{BO} \\
 & \textbf{($\sim$50)} & \textbf{(1000)} & \textbf{(1000)} & \textbf{(1000)} \\
\midrule
\texttt{mcf}     & \textbf{0.6141} & 0.5941 & 0.6120 & 0.6112 \\
\texttt{lbm}     & 0.5771 & 0.5752 & 0.5854 & \textbf{0.5858} \\
\texttt{omnetpp} & 0.3166 & 0.3176 & \textbf{0.3193} & 0.3181 \\
\bottomrule
\end{tabular}
\end{table}

Table~\ref{tab:champsim-per-workload} reports best IPC per method at maximum budget (mean across 3 seeds, with the cache-hierarchy constraint enforced post-hoc on samples that violated it). Three observations:

\textbf{\sysname{} reaches the IPC frontier on \texttt{mcf} fastest.} mcf is the most memory-latency-bound of the three, where hardware intuition (large LLC + SHIP replacement, signature-path prefetcher at L2C, large ways for irregular access) is most decisive. \sysname{} reaches IPC 0.6141 in $\sim$50 calls. The point estimate is 0.34\% above GA's 0.6120 at 1000 calls, but this gap is below the noise floor of our 5\,M-instruction simulation window and we do not claim a strict win at 1000 calls; we claim that \sysname{} reaches GA-at-1000-calls quality at $\sim$5\% of the budget.

\textbf{Within $\sim$1.5\% on \texttt{lbm} and \texttt{omnetpp}.} GA and BO at 1000 calls edge out \sysname{} at $\sim$50 calls by 1.4\% on lbm and 0.9\% on omnetpp, both within typical short-window simulation noise. \sysname{} achieves $\ge$98\% of the best baseline IPC at 5\% of the budget.

\textbf{Sample-efficiency budget scan.} Table~\ref{tab:champsim-budget-scan} reports the minimum budget at which \sysname{} matches Random@1000 calls' IPC---a tight \emph{equal-quality} comparison. \sysname{} reaches Random's 1000-call IPC in 20 calls on mcf (50$\times$) and 50 calls on lbm (20$\times$); on omnetpp, all four methods cluster within 0.002 IPC at all budgets, so the workload doesn't differentiate methods.

\begin{table}[t]
\small
\caption{Calls needed for \sysname{} to match Random's IPC at 1000 calls. Lower is better.}
\label{tab:champsim-budget-scan}
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Workload} & \textbf{Random@1000 IPC} & \textbf{\sysname{} budget} & \textbf{Speedup } \\
\midrule
\texttt{mcf}     & 0.594 & \textbf{20 calls}  & 50$\times$ \\
\texttt{lbm}     & 0.575 & \textbf{50 calls}  & 20$\times$ \\
\texttt{omnetpp} & 0.318 & noise zone         & --- \\
\bottomrule
\end{tabular}
\end{table}

The speedup column compares against uniform random search at its full 1000-call budget. The stricter, fairer comparison is at every method's own convergence point, defined as the smallest call count at which the best IPC has not improved by $>$10$^{-4}$ for the next 100 valid evaluations. Table~\ref{tab:champsim-convergence} shows the convergence-matched comparison.

\begin{table}[t]
\small
\caption{Calls to convergence (mean across 3 seeds) and convergence-matched sample-efficiency ratios. CC vs each baseline = baseline's convergence calls / CC's convergence calls.}
\label{tab:champsim-convergence}
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Workload} & \textbf{CC} & \textbf{Random} & \textbf{GA} & \textbf{BO} & \textbf{vs RS} & \textbf{vs GA} & \textbf{vs BO} \\
\midrule
\texttt{mcf}     & 55 & 464 & 543 & 621 & 8.5$\times$ & 9.9$\times$ & 11.4$\times$ \\
\texttt{lbm}     & 54 & 494 & 375 & 605 & 9.2$\times$ & 6.9$\times$ & 11.2$\times$ \\
\texttt{omnetpp} & 41 & 632 & 403 & 585 & 15.4$\times$ & 9.8$\times$ & 14.3$\times$ \\
\bottomrule
\end{tabular}
\end{table}

Convergence-matched, \sysname{}'s sample-efficiency advantage is \textbf{7--15$\times$} across the three workloads and three baselines, geometric mean $\approx$10$\times$. This is strictly more conservative than the 20--50$\times$ figure obtained against forced-1000-call baselines; we report it as the headline.

\textbf{Statistical caveat.} With $n=9$ paired observations (3 workloads $\times$ 3 seeds), a paired Wilcoxon signed-rank test does not detect statistically significant differences between CC and any baseline at $\alpha = 0.05$ \emph{at convergence-matched IPCs} (CC and GA/BO converge to overlapping bootstrap-95\% CIs on every workload; see supplementary stat\_tests.md). The right reading is that \sysname{} reaches a final-IPC indistinguishable from GA and BO, but reaches it an order of magnitude faster.

\subsection{Qualitative: hardware reasoning transfers}

We extracted Thinking/Action/Observation traces from each \sysname{} run by parsing the Claude session log into structured per-DSE-call records. Three behaviors echo what we observed on MAESTRO and confirm the methodology transfers:

\textbf{Workload-first reasoning.} Before the first evaluation, the agent reads the workload description, writes a multi-paragraph plan in \texttt{notes.md}, and picks the first config from that plan rather than from a uniform draw. On \texttt{mcf}, that plan correctly identifies the workload as latency-bound and prioritizes a 4\,MiB LLC with SHIP replacement plus an SPP prefetcher at L2.

\textbf{Intentional ablations.} On \texttt{mcf} seed~3, the agent removes the L2 prefetcher in call~2 to test whether call~1's gain is attributable to it (it is; IPC drops from 0.405 to 0.329). It then re-adds SPP at \emph{both} L2 and LLC in call~3 (IPC 0.414, the new best) and writes the insight to \texttt{notes.md}: ``\emph{High MPKI is not a harmful prefetcher for latency-bound workloads---evaluate by hits-saved-latency, not misses-caused.}'' This bandwidth-vs-latency-bound distinction is not given anywhere in the prompt or workspace files; it is derived from two data points by the agent itself.

\textbf{Implicit hierarchy prior.} 8 of 9 of \sysname{}'s best-IPC designs across the 9 grid runs satisfy the L1D~$\le$~L2C~$\le$~LLC hierarchy constraint without being told it; uniform-random samples violate it 15\% of the time. The agent has internalized monotonic memory hierarchies as a hardware-design prior, and largely respects it during search.

\subsection{Why does \sysname{} not strictly dominate on lbm/omnetpp?}

GA and BO at 1000 calls find slightly better configs on lbm and omnetpp than \sysname{} at $\sim$50 (margins of 1.4\% on lbm, 0.9\% on omnetpp). Both margins are within the noise floor of our 5\,M-instruction simulation window, so we caveat them as ``not statistically distinguishable from a tie'' rather than as strict losses. Two explanations are consistent with the point estimates: (i) for lbm (streaming, bandwidth-bound), the optimum involves moderate caches plus a single decisive prefetcher choice, an essentially low-dimensional sub-problem on which 1000 random-forest-guided proposals can plateau-search effectively; (ii) for omnetpp, the IPC distribution is sharply peaked---all methods land within 0.002 IPC, well inside short-window variance. The robust quantitative claim is therefore: \sysname{} at $\sim$50 calls reaches within 1--2\% of the best 1000-call gradient-free method on every workload, achieving comparable design quality at one-twentieth the simulator budget. The remaining within-noise differences require longer simulation (200M/500M instructions, DPC-3 standard) to resolve, which is the largest single follow-up our experimental design demands.

\subsection{What this experiment does and does not show}

We are explicit about the limits of this generalization test. ChampSim cache DSE is in Claude's training distribution: the SPP, SHIP, and hashed-perceptron papers cited in our \texttt{action\_space.md} appear verbatim in standard architecture corpora. Furthermore, \texttt{action\_space.md} contains a \emph{``Heuristics that usually work''} section with workload-specific guidance (e.g.\ ``mcf: large LLC + SHIP + SPP at L2''), which functions as a hand-curated retrieval database in static form. The fair statement of our finding is therefore: \emph{given a high-quality prompt that distills hardware-architecture priors, a coding agent can reach competitive cache-DSE designs in $\sim$50 simulator calls while transparently exposing its reasoning}; we do \emph{not} claim that this demonstrates open-domain generalization beyond cache-architecture problems. A stronger generalization test on a domain less covered by Claude's training data (e.g., NoC topology design or DRAM controller policies under non-standard objectives) is the natural next step and is left to future work. We also have not yet ablated \texttt{action\_space.md} with the heuristics removed; the headline numbers are conditional on the prompt as written.


==> backup_explainability.tex <==
\section{Explainability and Reward Hacks}
\label{sec:explainability}

A unique byproduct of agent-driven DSE is the reasoning trace in \texttt{notes.md}.
Unlike RL weight updates or GA population statistics, this trace provides human-readable explanations for each design decision.

\subsection{Example: Tile Size Discovery}

On the BERT Q-projection workload (K=C=768, X=512), the agent's trace includes:

\begin{quote}
\small\textit{``Call 6: Reducing L1 tiles from 768 to 16 dropped runtime from 150M to 1.17M cycles---a 128$\times$ improvement. Hypothesis: with 768-tile, the entire K dimension is serialized in one PE; with 16-tile, work is distributed across 768/16=48 effective parallel groups.''}
\end{quote}

This is a directly actionable insight for hardware architects: it identifies the specific bottleneck (tile-induced serialization) and suggests the design principle (tile size should enable parallel distribution).

\subsection{Detecting Reward Hacks}
\label{sec:reward-hacks}

More importantly, the agent's reasoning surfaces \textbf{simulator reward hacks}---configurations that exploit modeling artifacts rather than reflecting genuine hardware advantages.

In our BERT experiments, the agent discovered that setting \texttt{cluster\_l2=Y} when \texttt{Y=1} reduced energy by 14\% without changing runtime.
Its trace explains:

\begin{quote}
\small\textit{``With Y=1, SpatialMap on Y is degenerate---there is nothing to parallelize. But MAESTRO's energy model still skips the L2 multicast cost, producing an artificial energy reduction. This is a simulator artifact, not a real hardware improvement.''}
\end{quote}

This type of insight is impossible to extract from RL training curves or GA fitness trajectories.
ArchAgent~\cite{archagent} independently observed a similar phenomenon, calling them ``simulator escapes'' in the context of cache replacement policies.
We argue that \emph{interpretable optimization traces are not just a nice-to-have but a necessary tool for validating DSE results}, especially as the community moves toward increasingly automated architecture exploration~\cite{alphazero-moment}.


==> backup_related_works.tex <==
\section{Background}
\label{sec:background}

This section provides background on hardware DSE paradigms, coding agents as optimization interfaces, and the simulator families used in our evaluation.

\textbf{Traditional DSE.}
Random search, genetic algorithms~\cite{kao2020gamma}, Bayesian optimization~\cite{bo-dnn-mapping}, and simulated annealing have been widely used for hardware DSE.
ArchGym~\cite{archgym} provides a unified gym environment for comparing these methods.
These approaches treat the design space as a black box and require 10K--100K+ evaluations.

\textbf{RL for Hardware.}
Single-agent and multi-agent RL have been applied to DNN mapping~\cite{kao2020gamma}, NoC design, and memory hierarchy optimization.
While RL can learn effective policies, it requires extensive training (50K--200K steps in our experiments) and produces opaque policies.

\textbf{LLMs for Hardware Design.}
gem5~Co-Pilot~\cite{gem5copilot} uses GPT-4o with a pre-computed Design Space Database (DSDB) for CPU cache DSE, achieving near-optimal results in 1--8 simulations.
However, it relies heavily on the DSDB (7,770 pre-computed configurations) for retrieval-augmented generation.
LLM-DSE~\cite{llmdse} coordinates four specialized LLM agents for HLS directive optimization, achieving 2.55$\times$ gains over prior methods.
ArchAgent~\cite{archagent} uses agentic AI to discover novel cache replacement policies and identifies ``simulator escapes'' where the AI exploits simulation artifacts.
Our work differs from all three in requiring \emph{no pre-computed database, no custom multi-agent framework, and no domain-specific fine-tuning}---only a coding agent and a simulator script.

\textbf{Vision.}
Sankaralingam~\cite{alphazero-moment} argues for ``automated idea factories'' that systematically explore architecture design spaces, drawing parallels to AlphaZero's impact on game-playing.
\sysname{} represents a concrete instantiation of this vision for DSE, demonstrating that current coding agents already possess sufficient reasoning capability for practical hardware optimization.
